ASAS-SN follow-up of IceCube high-energy neutrino alerts

We report on the search for optical counterparts to IceCube neutrino alerts released between April 2016 and August 2021 with the All-Sky Automated Survey for SuperNovae (ASAS-SN). Despite the discovery of a diffuse astrophysical high-energy neutrino flux in 2013, the source of those neutrinos remains largely unknown. Since 2016, IceCube has published likely-astrophysical neutrinos as public realtime alerts. Through a combination of normal survey and triggered target-of-opportunity observations, ASAS-SN obtained images within 1 hour of the neutrino detection for 20% (11) of all observable IceCube alerts and within one day for another 57% (32). For all observable alerts, we obtained images within at least two weeks from the neutrino alert. ASAS-SN provides the only optical follow-up for about 17% of IceCube's neutrino alerts. We recover the two previously claimed counterparts to neutrino alerts, the flaring-blazar TXS 0506+056 and the tidal disruption event AT2019dsg. We investigate the light curves of previously-detected transients in the alert footprints, but do not identify any further candidate neutrino sources. We also analysed the optical light curves of Fermi 4FGL sources coincident with high-energy neutrino alerts, but do not identify any contemporaneous flaring activity. Finally, we derive constraints on the luminosity functions of neutrino sources for a range of assumed evolution models.

==> ASAS-SN Neutrino Follow-up Paper with tracking/latex/alert_table_not_observed.tex <==
	 IC160806A & 122.81 & $-0.81$ & 0.0 & proximity to sun & \cite{ic160806a} \\ 
	 IC171015A & 162.86 & $-15.44$ & 14.9 & proximity to sun & \cite{ic171015a} \\ 
	 IC180908A & 144.58 & $-2.13$ & 6.3 & proximity to sun & \cite{ic180908a} \\ 
	 IC181014A & 225.15 & $-34.80$ & 10.5 & proximity to sun & \cite{ic181014a} \\ 
	 IC190124A & 307.4 & $-32.18$ & 2.0 & proximity to sun & \cite{ic190124a} \\ 
	 IC190819A & 148.8 & $+1.38$ & 9.3 & proximity to sun & \cite{ic190819a} \\ 
	 IC190922A & 167.43 & $-22.39$ & 32.2 & proximity to sun & \cite{ic190922a} \\ 
	 IC191119A & 230.1 & $+3.17$ & 61.2 & proximity to sun & \cite{ic191119a} \\ 
	 IC200421A & 87.93 & $+8.23$ & 24.4 & operation & \cite{ic200421a} \\ 
	 IC200806A & 157.25 & $+47.75$ & 1.8 & proximity to sun & \cite{ic200806a} \\ 
	 IC200921A & 195.29 & $+26.24$ & 12.0 & proximity to sun & \cite{ic200921a} \\ 
	 IC200926B & 184.75 & $+32.93$ & 9.0 & proximity to sun & \cite{ic200926b} \\ 
	 IC201014A & 221.22 & $+14.44$ & 1.9 & proximity to sun & \cite{ic201014a} \\ 
	 IC210516A & 91.76 & $+9.52$ & 2.2 & proximity to sun & \cite{ic210516a} \\ 
	 IC210730A & 105.73 & $+14.79$ & 6.6 & proximity to sun & \cite{ic210730a} \\ 


==> ASAS-SN Neutrino Follow-up Paper with tracking/latex/alert_table_observed.tex <==
IC160427A & 240.57 & $+9.34$ & 1.4 & 100.0 & 100.0 & - & \cite{ic160427a} \\ 
IC160731A & 214.50 & $-0.33$ & 2.2 & 36.2 & 100.0 & 85 & - \\ 
IC160814A & 200.30 & $-32.40$ & 12.0 & 0.0 & 100.0 & - & \cite{ic160814a} \\ 
IC161103A & 40.83 & $+12.56$ & 3.1 & 79.9 & 100.0 & - & \cite{ic161103a} \\ 
IC161210A & 46.58 & $+14.98$ & 1.7 & 0.0 & 100.0 & 49 & \cite{ic161210a} \\ 
IC170312A & 305.15 & $-26.61$ & 0.9 & 0.0 & 100.0 & - & \cite{ic170312a} \\ 
IC170321A & 98.30 & $-15.02$ & 5.6 & 4.5 & 100.0 & 28 & \cite{ic170321a} \\ 
IC170922A & 77.43 & $+5.72$ & 1.3 & 100.0 & 100.0 & 57 & \cite{ic170922a} \\ 
IC171106A & 340.00 & $+7.40$ & 0.7 & 100.0 & 100.0 & 75 & \cite{ic171106a} \\ 
IC181023A & 270.18 & $-8.57$ & 9.3 & 70.5 & 100.0 & 28 & \cite{ic181023a} \\ 
IC190104A & 357.98 & $-26.65$ & 18.5 & 14.0 & 100.0 & - & \cite{ic190104a} \\ 
IC190221A & 268.81 & $-17.04$ & 5.2 & 78.6 & 100.0 & - & \cite{ic190221a} \\ 
IC190331A & 337.68 & $-20.70$ & 0.4 & 0.0 & 100.0 & - & \cite{ic190331a} \\ 
IC190503A & 120.28 & $+6.35$ & 1.9 & 100.0 & 100.0 & 36 & \cite{ic190503a} \\ 
IC190619A & 343.26 & $+10.73$ & 27.2 & 100.0 & 100.0 & 55 & \cite{ic190619a} \\ 
IC190629A & 27.22 & $+84.33$ & 5.0 & 0.0 & 70.6 & 34 & \cite{ic190629a} \\ 
IC190704A & 161.85 & $+27.11$ & 21.0 & 100.0 & 100.0 & 49 & \cite{ic190704a} \\ 
IC190712A & 76.46 & $+13.06$ & 92.0 & 0.0 & 13.1 & 30 & \cite{ic190712a} \\ 
IC190730A & 225.79 & $+10.47$ & 5.4 & 100.0 & 100.0 & 67 & \cite{ic190730a} \\ 
IC190922B & 5.76 & $-1.57$ & 4.5 & 100.0 & 100.0 & 51 & \cite{ic190922b} \\ 
IC191001A & 314.08 & $+12.94$ & 25.5 & 100.0 & 100.0 & 59 & \cite{ic191001a} \\ 
IC191122A & 27.25 & $-0.04$ & 12.2 & 100.0 & 100.0 & 33 & \cite{ic191122a} \\ 
IC191204A & 79.72 & $+2.80$ & 11.6 & 98.8 & 100.0 & 33 & \cite{ic191204a} \\ 
IC191215A & 285.87 & $+58.92$ & 12.8 & 0.0 & 12.4 & 47 & \cite{ic191215a} \\ 
IC191231A & 46.36 & $+20.42$ & 35.6 & 100.0 & 100.0 & 46 & \cite{ic191231a} \\ 
IC200107A & 148.18 & $+35.46$ & 7.6 & 0.0 & 78.2 & 50$^{*}$ & \cite{ic200107a} \\ 
IC200109A & 164.49 & $+11.87$ & 22.5 & 77.7 & 100.0 & 77 & \cite{ic200109a} \\ 
IC200117A & 116.24 & $+29.14$ & 2.9 & 0.0 & 100.0 & 38 & \cite{ic200117a} \\ 
IC200410A & 242.58 & $+11.61$ & 377.9 & 38.0 & 100.0 & 31 & \cite{ic200410a} \\ 
IC200425A & 100.10 & $+53.57$ & 18.8 & 7.2 & 100.0 & 48 & \cite{ic200425a} \\ 
IC200512A & 295.18 & $+15.79$ & 9.8 & 62.5 & 100.0 & 32 & \cite{ic200512a} \\ 
IC200523A & 338.64 & $+1.75$ & 90.6 & 24.5 & 100.0 & 25 & \cite{ic200523a} \\ 
IC200530A & 255.37 & $+26.61$ & 25.3 & 92.4 & 100.0 & 59 & \cite{ic200530a} \\ 
IC200614A & 33.84 & $+31.61$ & 47.8 & 35.2 & 100.0 & 42 & \cite{ic200614a} \\ 
IC200615A & 142.95 & $+3.66$ & 5.9 & 97.9 & 100.0 & 83 & \cite{ic200615a} \\ 
IC200620A & 162.11 & $+11.95$ & 1.7 & 100.0 & 100.0 & 32 & \cite{ic200620a} \\ 
IC200911A & 51.11 & $+38.11$ & 52.7 & 46.5 & 100.0 & 41 & \cite{ic200911a} \\ 
IC200916A & 109.78 & $+14.36$ & 4.2 & 100.0 & 100.0 & 32 & \cite{ic200916a} \\ 
IC200926A & 96.46 & $-4.33$ & 1.7 & 100.0 & 100.0 & 44 & \cite{ic200926a} \\ 
IC200929A & 29.53 & $+3.47$ & 1.1 & 65.1 & 100.0 & 47 & \cite{ic200929a} \\ 
IC201007A & 265.17 & $+5.34$ & 0.6 & 0.0 & 100.0 & 88 & \cite{ic201007a} \\ 
IC201021A & 260.82 & $+14.55$ & 6.9 & 2.6 & 100.0 & 30 & \cite{ic201021a} \\ 
IC201114A & 105.25 & $+6.05$ & 4.5 & 100.0 & 100.0 & 56 & \cite{ic201114a} \\ 
IC201115A & 195.12 & $+1.38$ & 6.6 & 0.0 & 100.0 & 46 & \cite{ic201115a} \\ 
IC201120A & 307.53 & $+40.77$ & 64.3 & 82.5 & 100.0 & 50 & \cite{ic201120a} \\ 
IC201130A & 30.54 & $-12.10$ & 5.4 & 100.0 & 100.0 & 15 & \cite{ic201130a} \\ 
IC201209A & 6.86 & $-9.25$ & 4.7 & 100.0 & 100.0 & 19 & \cite{ic201209a} \\ 
IC201221A & 261.69 & $+41.81$ & 8.9 & 0.0 & 100.0 & 56 & \cite{ic201221a} \\ 
IC201222A & 206.37 & $+13.44$ & 1.5 & 100.0 & 100.0 & 53 & \cite{ic201222a} \\ 
IC210210A & 206.06 & $+4.78$ & 2.8 & 100.0 & 100.0 & 65 & \cite{ic210210a} \\ 
IC210503A & 143.53 & $+41.81$ & 102.6 & 27.1 & 100.0 & 41 & \cite{ic210503a} \\ 
IC210510A & 268.42 & $+3.81$ & 4.0 & 0.0 & 100.0 & 28 & \cite{ic210510a} \\ 
IC210608A & 337.41 & $+18.37$ & 109.7 & 94.8 & 100.0 & 31 & \cite{ic210608a} \\ 
IC210629A & 340.75 & $+12.94$ & 6.0 & 100.0 & 100.0 & 35 & \cite{ic210629a} \\ 
IC210717A & 46.49 & $-1.34$ & 30.0 & 69.2 & 100.0 & 50$^{*}$ & \cite{ic210717a} \\ 
IC210811A & 270.79 & $+25.28$ & 3.2 & 100.0 & 100.0 & 66 & \cite{ic210811a} \\ 

